Gradient-Based Trajectory Optimization With Learned Dynamics

Trajectory optimization methods have achieved an exceptional level of performance on real-world robots in recent years. These methods heavily rely on accurate analytical models of the dynamics, yet some aspects of the physical world can only be captured to a limited extent. An alternative approach is to leverage machine learning techniques to learn a differentiable dynamics model of the system from data. In this work, we use trajectory optimization and model learning for performing highly dynamic and complex tasks with robotic systems in absence of accurate analytical models of the dynamics. We show that a neural network can model highly nonlinear behaviors accurately for large time horizons, from data collected in only 25 minutes of interactions on two distinct robots: (i) the Boston Dynamics Spot and an (ii) RC car. Furthermore, we use the gradients of the neural network to perform gradient-based trajectory optimization. In our hardware experiments, we demonstrate that our learned model can represent complex dynamics for both the Spot and Radio-controlled (RC) car, and gives good performance in combination with trajectory optimization methods.

==> chapters/analysis.tex <==


\section{Model Selection}
\label{sec:model_selection}
%\begin{comment}
\looseness=-1
In this section, we describe the model selection process. 
We used our simulated car model to evaluate different neural network architectures on synthetic data. 
While network training solely relies on a loss over one time step, our goal is to learn a model that can match the dynamics of the car over an entire trajectory. 
To evaluate this performance, we use 40 prerecorded validation trajectories with known end state poses. 
We infer the corresponding control trajectories on each learned model candidate and compare the resulting end-state poses by computing the final state error.
We denote the mean of all 40 final pose errors %per model candidate 
as \emph{Trajectory Validation Error} (in short TVE), i.e.
%
\begin{equation}
    \mathrm{TVE} = \frac{1}{40} \sum_{j = 0}^{40} \norm{\hat{\x}_n - \x^j_n}_1,
    \label{eq:TVE}
\end{equation}
%
where $\x^j_n$ denotes the final state of a particular validation trajectory $j$.
We use this as a metric to evaluate the efficacy of the different neural network architectures.
We note that other evaluation metrics could also be applied, but we find that this one works well for our use case, as it essentially captures the accumulated state error throughout the trajectory.


\subsection{Loss Function}

During neural network training, choosing a suitable loss function is of utmost importance. Since we train on the relative velocities of the car, we encounter a high dynamic range. We expect that the most suitable models for trajectory inference are those that minimize the relative error of the training data. Our intuition is that the loss function should be more sensitive to absolute errors for small velocities. We tackle this by introducing the following relative loss for our training:

\begin{equation}
\label{eq:relative_loss}
    L_{rel}(\theta) = \frac{\norm{ \v_{i+1} -  \f_{\theta}(\v_i, \u_i) }_1}{\norm{\v_{i+1} }_1+\epsilon},
\end{equation}

where $\epsilon > 0$ prevents numerical problems for small velocities. 
%
%\BS{Think this needs to be explained better. So what do you mean with high dynamic range?}
%\NK{Essentially: the loss is relative to the magnitude of the sample. For example, for a low velocity of 0.01, 0.015 is 50 percent off. For a high velocity of 1, 1.005 is relatively more accurate, even though the absolute difference is the same. Both L1 and L2 loss would assign the same loss value for both examples, while our relative loss does not. I agree it should be explained better and with a better formula. BTW: the epsilon is necessary to not let the loss explode for very small values. Plus there is some noise in the data.}
%
%where $y_k$ is a noisy measurement of the true transition $f(x_k,u_k)$~\cref{eq:trajectoryOptimizationProblem_Dynamics}, i.e., $y_k = f(x_k,u_k) + \epsilon_k$.
%
\begin{figure} %[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/loss_traj_comparisons/v2/loss_traj_comparisons.pdf}
    \caption{ Left: Comaprison of distribution for TVE of different model architectures trained with respect to $L1$, $L2$ and $L_{rel}$ (Eq. (\ref{eq:relative_loss})) training losses. 
    Right: Comparison of different model architectures with \gls{relu} or \gls{gelu} activations on the $L_{rel}$  loss and TVE (Eq. (\ref{eq:TVE})).}
    
    %Comparison between model architectures with \gls{relu} and \gls{gelu} activations for different training losses $L1$, $L2$ and $L_{rel}$(~\cref{eq:relative_loss_v2}). }
    %\NK{This plot shows that ReLU and GeLU perform well, that ReLU is a bit better on average, but there are many good GeLU models. Also it shows that while Loss and performance on validation trajectories correlates, it is very important to look at validation trajectories when picking a model. Then it shows that both L1 loss and relative loss perform well enough, and that dynamic weighting helps.}}
    \label{fig:validation_traj_vs_loss}
\end{figure}
%
We trained 15 multiple feed-forward and fully connected neural networks with 8 hidden layers and 64 neurons per layer with three loss functions: L1 loss, L2 loss and our relative loss. For each network, we inferred the validation trajectories and calculated the mean end distance (see \cref{fig:validation_traj_vs_loss} on the left). We found that networks trained with either L1 loss or relative loss perform notably better than those trained with L2 loss. Due to the lower variance, we use our relative loss for all further training.

\subsection{Activation Functions and Network Size} \label{activation_function}

Activation functions are used to capture nonlinearities with neural networks. Typical choices for activation functions are sigmoid, $\tanh$, and \gls{relu}. Nevertheless, sigmoid and $\tanh$ often suffer from the well-known exploding/vanishing gradients problem when trained with backpropogation~\cite{Hochreiter91}. To this end, \gls{relu} is mostly preferred in the machine learning community. However, the gradient of \gls{relu} is not continuous, which potentially imposes a challenge for gradient-based trajectory optimization. Particularly a neural network with \gls{relu} activations may result in very noisy (i.e. fluctuating) control sequences when employed with trajectory optimization. 
%as depicted in \cref{fig:smoothness}, a neural network with \gls{relu} activations, results in very noisy (i.e. fluctuating) input sequences. 
As we want to apply the optimized control inputs directly to our physical system, this can have a negative impact on the overall performance, and could potentially even damage the hardware.
Therefore, in this work, we also consider \gls{gelu}~\cite{GELU} as a differentiable alternative to \gls{relu}. 
We hypothesize that because \gls{gelu} has continuous gradients, it could result in smoother control trajectories, which would make it better suited for our application.
We further discuss this matter in~\cref{sec:discussion}.

%Therefore, we believe that \gls{gelu} would be better suited for our application. We validate this hypothesis in \cref{gradientsmoothness}.
%As visualized in \cref{fig:smoothness}, a neural network with \gls{gelu} activations returns considerably smoother input sequences, which can seamlessly be applied to the physical car.

%\NK{Concerning the flow of argumentation: I would prefer to at this point just mention that we explore ReLU and GELU. ReLU because it is ubiquitous, GELU because the gradient is continuous.
%Then later on, when we go into results of trajectory optimization, show that indeed GELU is much better, so then confirm the choice.}

%Therefore, in this work, we also consider its differentiable counterpart \gls{gelu}~\cite{GELU}. Particularly, since \gls{gelu} is differentiable, we expect a neural network with \gls{gelu}, instead of \gls{relu}, to provide smoother trajectories (input sequences) when combined with our trajectory optimization scheme. Since, we apply the optimized inputs on a hardware platform, it is extremely important that the sequence is smooth to avoid damage to the motors.
%\NK{talk about activation functions, that we intuitively want a smooth one, that ReLU performs well, that GELU might as well.}

For selecting the network architecture (activation functions and size), we trained a total of over 200 neural networks of different sizes with both ReLU and GELU as activation functions (see \cref{fig:validation_traj_vs_loss} on the right). Furthermore,  we performed a grid search with different network sizes for both activation functions (\cref{fig:grid_search}).
Finally, we selected an architecture with 8 hidden layers of 64 neurons each with the GELU activation function based on two criteria \emph{(i)} network size/evaluation time, and \emph{(ii)} performance on TVE and test loss. %\BS{Hereby, we noticed that the test loss of a network is only loosely correlated with TVE, further confirming the utility of a metric based on more than a single trajectory step.
%Additionally, we conclude that while ReLU performs better in general \SZ{in general means for other types of problems? better in what way?}, our best performing models, both in terms of TVE and the test loss, are those that utilize the GELU activation function.}
%\SZ{Refer to the grid, network size / eval time VS performance}
\begin{comment}
    \subsection{Dynamic Sample Weighting}
    
    While exploring the dynamics of models with a low test loss, but high mean validation trajectory distance, we found that these settings typically overemphasize static or quasi-static behavior. This is based on the fact that predicting no change in velocity is a good initial guess for many data points in the training set.
    However, we are interested in learning a model that can accurately capture \emph{dynamic} behavior. To emphasize this, we rate "how dynamic" each data point is, then weigh the loss of each data point with this constant. \NK{do we need formulas? do we even have space for them?}
    \SZ{I would try to briefly explain it with words}
    To analyze this, we trained 15 networks both without and with dynamic weighting (\cref{fig:validation_traj_vs_loss}, right). We conclude that networks trained with dynamic weighting perform better on the validation trajectories.
    \BS{Maybe explain more? Could be a contribution in the end.}
    \NK{I agree, on slack I wrote more details.}
\end{comment}
%\subsection{Network Size}
\begin{figure} [h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/grid_relu_gelu/v2/grid_relu_gelu.pdf}
    \caption{Results from grid search for different network architectures with \gls{relu} or \gls{gelu} activations based on TVE (Eq. (\ref{eq:TVE})).}%\NK{Draft: Results of grid search, show best loss and best traj mean - for both Relu and Gelu}}
    \label{fig:grid_search}
\end{figure}
%While larger neural networks can be more expressive, they have a higher risk of over-fitting. Additionally, they are computationally more expensive, which can be prohibitive when used in online trajectory optimization. Therefore, our goal is to choose a network size as small as possible while still capturing the dynamic behavior of the \gls{rc} car. To this end, we performed a grid search where we trained 5 musingboth dusins of hidden layers and neurons per layer, using both ReLU and GELU activation functions (\cref{fig:grid_search}). Of those 5 models, we pick the best one based on the TVE.
%While ReLU performs better for smaller networks, we achieve again good performance with the GELU activation function. %We choose 8 hidden layers with 64 neurons each as a good trade-off between network size and performance.

%In summary, for our real \gls{rc} car, we choose fully connected feed-forward networks with 8 hidden layers of 64 neurons each with the GELU activation function. We train the networks with our relative loss function, weighting each sample based on how dynamic it is. We train multiple models and select one based on the mean validation trajectory distance.
    




==> figures/scenarios/Drifting_Turn.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00,0.0,1.0}%
\definecolor{mycolor2}{rgb}{1.00,0.0,0.0}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.519in,
height=1.492in,
at={(0.758in,2.553in)},
scale only axis,
xmin=0,
xmax=60,
ymin=-4.2,
ymax=4.2,
ylabel style={font=\color{white!15!black}},
ylabel={Local velocities},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.99,0.95)}, font=\LARGE, anchor=north east, legend cell align=left, align=left, draw=white!15!black},
title style={font=\huge},xlabel style={font=\LARGE},ylabel style={font=\LARGE},xticklabel style={font=\LARGE},yticklabel style={font=\LARGE}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	0.00276613980531693\\
2	0.00823767855763435\\
3	0.0119603611528873\\
4	0.0065997987985611\\
5	-0.0087086856365204\\
6	-0.0284667871892452\\
7	-0.0463894754648208\\
8	-0.0569241866469385\\
9	-0.060579590499401\\
10	-0.060689952224493\\
11	-0.060554835945368\\
12	-0.061766803264618\\
13	-0.0640689209103585\\
14	-0.066185016185045\\
15	-0.0668968074023725\\
16	-0.0671349093317985\\
17	-0.071399509906769\\
18	-0.072746481746435\\
19	-0.051424540579319\\
20	-0.0101034343242646\\
21	0.0317312031984329\\
22	0.0372432544827461\\
23	0.0745005905628205\\
24	0.255367085337639\\
25	0.564088616520165\\
26	0.90141098946333\\
27	1.15962199866771\\
28	1.24598857015372\\
29	1.21318805962801\\
30	1.16702847182751\\
31	1.11253626644611\\
32	1.08980633318424\\
33	1.00398447364569\\
34	0.86630154401064\\
35	0.69597791880369\\
36	0.443265298381448\\
37	0.182736720889806\\
38	0.078078266233206\\
39	-0.00553730875253675\\
40	-0.0820181518793105\\
41	-0.102459043264389\\
42	-0.0876626931130885\\
43	-0.0840194150805475\\
44	-0.072905458509922\\
45	-0.063912682235241\\
46	-0.071172025054693\\
47	-0.0854314863681795\\
48	-0.0888616964221\\
49	-0.0770220905542375\\
50	-0.0584452226758005\\
51	-0.0375859066843987\\
52	-0.0122221000492573\\
53	0.0184967368841172\\
54	0.0466695986688137\\
55	0.056427363306284\\
56	0.0430748797953129\\
57	0.0147678516805172\\
58	-0.0118589960038662\\
59	-0.0228599645197392\\
60	-0.0265559926629067\\
};
\addlegendentry{$v_{x} [m/s]$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.281276693567634\\
2	-0.56187015026808\\
3	-0.85024371743202\\
4	-1.14116191864013\\
5	-1.42644323408603\\
6	-1.70181266963482\\
7	-1.96788690984249\\
8	-2.22337894141674\\
9	-2.4664818495512\\
10	-2.69422061741352\\
11	-2.90371723473072\\
12	-3.09335432946682\\
13	-3.26302081346512\\
14	-3.41365702450276\\
15	-3.54671381413936\\
16	-3.66366483271122\\
17	-3.76411065459251\\
18	-3.84189695119858\\
19	-3.89123842120171\\
20	-3.91674309968948\\
21	-3.92785549163818\\
22	-3.79279017448426\\
23	-3.55351947247982\\
24	-3.2374070584774\\
25	-2.8457198292017\\
26	-2.38505937159062\\
27	-1.86046242713928\\
28	-1.35640807449818\\
29	-1.07392318546772\\
30	-0.95373574644327\\
31	-0.909708961844445\\
32	-0.92112109065056\\
33	-1.03110194206238\\
34	-1.20844267308712\\
35	-1.43430210649967\\
36	-1.68627820909024\\
37	-1.67198270559311\\
38	-1.5887975692749\\
39	-1.44379768520594\\
40	-1.22997634112835\\
41	-0.99614314734936\\
42	-0.77638193964958\\
43	-0.59114634990692\\
44	-0.488128960132599\\
45	-0.548293702304365\\
46	-0.764593966305255\\
47	-1.0202919691801\\
48	-1.27156231552363\\
49	-1.5110021084547\\
50	-1.72994211316109\\
51	-1.92791685461998\\
52	-2.11837783455849\\
53	-2.31036588549614\\
54	-2.5006952136755\\
55	-2.680619135499\\
56	-2.85551078617573\\
57	-3.02666835486889\\
58	-3.19150038063526\\
59	-3.34730520844459\\
60	-3.49051617085934\\
};
\addlegendentry{$v_{y} [m/s]$}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.0267043244093657\\
2	-0.115502402186394\\
3	-0.24972902610898\\
4	-0.375976413488388\\
5	-0.458290195092559\\
6	-0.492186360061169\\
7	-0.490981936454773\\
8	-0.463596163317561\\
9	-0.419269502162934\\
10	-0.366861233487725\\
11	-0.31096413731575\\
12	-0.251142885535955\\
13	-0.184937166050077\\
14	-0.112427836284042\\
15	-0.0380669161677361\\
16	0.0442803930491209\\
17	0.192030100151897\\
18	0.446366099640727\\
19	0.696799233555795\\
20	0.835533812642095\\
21	0.870285741984845\\
22	0.89281875640154\\
23	1.13955985754728\\
24	1.64016019552946\\
25	2.17718660831452\\
26	2.59513847529888\\
27	2.82506950199604\\
28	2.79334433376789\\
29	2.62684151530266\\
30	2.50475630164147\\
31	2.25816808640957\\
32	1.53325740247965\\
33	0.597417019307615\\
34	-0.313043268397451\\
35	-1.03341959416867\\
36	-1.59657720476389\\
37	-1.46401539444923\\
38	-0.8861331269145\\
39	-0.245408043265342\\
40	0.295026591047645\\
41	0.64158171415329\\
42	0.69896288216114\\
43	0.525672510266305\\
44	0.377431875094771\\
45	0.345622999593615\\
46	0.423156330361962\\
47	0.62254920601845\\
48	0.879580713808535\\
49	1.09094202518463\\
50	1.19949650019407\\
51	1.21344555169344\\
52	1.16565763950348\\
53	1.07660852372647\\
54	0.947041623294355\\
55	0.77236656099558\\
56	0.57685498148203\\
57	0.408353051170707\\
58	0.289991302415729\\
59	0.160361593589187\\
60	-0.00252694822847843\\
};
\addlegendentry{$v_{\theta} [rad/s]$}

\end{axis}

\begin{axis}[%
width=4.519in,
height=1.492in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=60,
xlabel style={font=\color{white!15!black}},
xlabel={Step},
ymin=-1.2,
ymax=1.2,
ylabel style={font=\color{white!15!black}},
ylabel={Control},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.99,0.95)}, font=\LARGE, anchor=north east, legend cell align=left, align=left, draw=white!15!black},
title style={font=\huge},xlabel style={font=\LARGE},ylabel style={font=\LARGE},xticklabel style={font=\LARGE},yticklabel style={font=\LARGE}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	0.509089021449919\\
2	0.74253040117299\\
3	0.841191104241941\\
4	0.886315409946536\\
5	0.92095034424346\\
6	0.956700935101247\\
7	0.987954327242122\\
8	1\\
9	1\\
10	1\\
11	1\\
12	1\\
13	1\\
14	1\\
15	1\\
16	1\\
17	1\\
18	1\\
19	1\\
20	1\\
21	0.966868553921359\\
22	0.552323131457752\\
23	0.158234111675472\\
24	-0.0699950117998446\\
25	-0.150116012282673\\
26	-0.13670063130333\\
27	-0.0136175946421217\\
28	0.251562937899566\\
29	0.613865960258859\\
30	0.883659258006621\\
31	0.999777665460363\\
32	0.999692840736955\\
33	0.949045901654286\\
34	0.87980806552411\\
35	0.947783721069663\\
36	1\\
37	0.421063486049685\\
38	0.2152311259911\\
39	0.127246091886116\\
40	0.0500644889843327\\
41	-0.0161062769772384\\
42	-0.0164995104226479\\
43	0.0701596425948676\\
44	0.205210177689038\\
45	0.349251049678525\\
46	0.504985446220987\\
47	0.662459122778746\\
48	0.784819837446556\\
49	0.856117542334859\\
50	0.886659670600428\\
51	0.902951904689054\\
52	0.927537008545596\\
53	0.963175620165764\\
54	0.99645859064908\\
55	1\\
56	1\\
57	1\\
58	1\\
59	1\\
60	1\\
};
\addlegendentry{$u_{steer}$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.174556451874426\\
2	-0.272601378318049\\
3	-0.314645084020584\\
4	-0.323083053041482\\
5	-0.314862582059026\\
6	-0.299720768341331\\
7	-0.281476888468582\\
8	-0.260574448230597\\
9	-0.235743917668366\\
10	-0.206142780005103\\
11	-0.171914884690324\\
12	-0.133876363608816\\
13	-0.0930404611005103\\
14	-0.0501603758817143\\
15	-0.00559593709107229\\
16	0.0403287255973421\\
17	0.0874882430454474\\
18	0.139651819877035\\
19	0.212343005569378\\
20	0.326356758658649\\
21	0.469977957694125\\
22	0.592316404308054\\
23	0.645220332627915\\
24	0.696128103800129\\
25	0.733837955715795\\
26	0.738767766506041\\
27	0.708396610824733\\
28	0.630421978264852\\
29	0.486442457673854\\
30	0.254815230591881\\
31	-0.124192715149775\\
32	-0.663105254243261\\
33	-1\\
34	-1\\
35	-1\\
36	-1\\
37	-0.63501165278241\\
38	-0.257006901484933\\
39	0.0863529780659505\\
40	0.363768710021627\\
41	0.557609427018064\\
42	0.663246363313298\\
43	0.706272763505805\\
44	0.71753955578156\\
45	0.722096173295702\\
46	0.733237280461957\\
47	0.749103623014332\\
48	0.759554316086967\\
49	0.754954036982069\\
50	0.728521724986139\\
51	0.680229200475625\\
52	0.614616808567266\\
53	0.536957077742887\\
54	0.452409162675682\\
55	0.365378976367629\\
56	0.280875558483495\\
57	0.20491818781257\\
58	0.134691162764301\\
59	0.0483954408570988\\
60	-0.036934848653593\\
};
\addlegendentry{$u_{throttle}$}

\end{axis}
\end{tikzpicture}%

==> figures/scenarios/Dynamic_Reverse.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00,0.0,1.0}%
\definecolor{mycolor2}{rgb}{1.00,0.0,0.0}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.519in,
height=1.492in,
at={(0.758in,2.553in)},
scale only axis,
xmin=0,
xmax=40,
ymin=-4.2,
ymax=2.2,
ylabel style={font=\color{white!15!black}},
ylabel={Local velocities},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
title style={font=\huge},xlabel style={font=\LARGE},ylabel style={font=\LARGE},xticklabel style={font=\LARGE},yticklabel style={font=\LARGE}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	0.000323094427585602\\
2	-0.00116027891635895\\
3	-0.0019519217312336\\
4	-0.00337997451424599\\
5	-0.00473331660032273\\
6	-0.00717340037226675\\
7	-0.0114450417459011\\
8	-0.0169212743639946\\
9	-0.0219172239303589\\
10	-0.0249604135751724\\
11	-0.0262109376490116\\
12	-0.0273846834897995\\
13	-0.0301364623010159\\
14	-0.0348614528775215\\
15	-0.0404961034655571\\
16	-0.045679584145546\\
17	-0.0497642531991005\\
18	-0.0526348873972895\\
19	-0.0538158416748045\\
20	-0.0531080178916455\\
21	-0.050578471273184\\
22	-0.0497016124427319\\
23	-0.0441379845142365\\
24	-0.0510767474770545\\
25	-0.0882577523589135\\
26	-0.246975626796484\\
27	-0.550334081053735\\
28	-0.918614342808725\\
29	-1.25071920454502\\
30	-1.43859185278416\\
31	-1.4018440246582\\
32	-1.17189846932888\\
33	-0.847928412258625\\
34	-0.50962843000889\\
35	-0.199147984385491\\
36	0.0489111989736557\\
37	0.105936974287033\\
38	0.114125590771436\\
39	0.084028635174036\\
40	0.0211667641997338\\
};
%\addlegendentry{$v_{x} [m/s]$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.0132157187908888\\
2	-0.0436879321932793\\
3	-0.09521272033453\\
4	-0.178368324413895\\
5	-0.306827919557691\\
6	-0.482240281999111\\
7	-0.697866417467595\\
8	-0.945580154657365\\
9	-1.213284060359\\
10	-1.48648895323276\\
11	-1.75608403980732\\
12	-2.0194461196661\\
13	-2.27416478097439\\
14	-2.51885913312435\\
15	-2.74749733507633\\
16	-2.95557841658592\\
17	-3.14270697534084\\
18	-3.30941878259182\\
19	-3.45721386373043\\
20	-3.58813919126988\\
21	-3.70421715080738\\
22	-3.80630403757096\\
23	-3.88557493686676\\
24	-3.81699576973915\\
25	-3.60784985125065\\
26	-3.27861316502094\\
27	-2.85016022622586\\
28	-2.343839854002\\
29	-1.73414178192616\\
30	-1.02485340088606\\
31	-0.321463281288743\\
32	0.241031181067229\\
33	0.63818905502558\\
34	0.91806046664715\\
35	1.08654230833054\\
36	1.15056283771992\\
37	1.18029244244099\\
38	1.20491590350866\\
39	1.15394622087479\\
40	1.06359276920557\\
};
%\addlegendentry{$v_{y} [m/s]$}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
1	0.00463030301034451\\
2	0.00560003332793715\\
3	0.00704010017216205\\
4	0.0073481071740389\\
5	0.0054341834038496\\
6	0.00216909684240818\\
7	0.000162385404109955\\
8	0.00143816694617272\\
9	0.0060945376753807\\
10	0.0111289601773024\\
11	0.0112489890307188\\
12	0.00344971194863319\\
13	-0.00899607315659525\\
14	-0.0191588792949915\\
15	-0.0208339188247919\\
16	-0.0128012895584106\\
17	0.00197519548237324\\
18	0.0198284815996886\\
19	0.0328799989074468\\
20	0.0285782944411039\\
21	-0.0119360256940127\\
22	-0.0892159435898065\\
23	-0.280742067843676\\
24	-0.604371819645165\\
25	-1.03020630776882\\
26	-1.55019845813513\\
27	-2.190573066473\\
28	-2.8238770365715\\
29	-3.35922338068485\\
30	-3.70505422353745\\
31	-3.61459694802761\\
32	-2.96130560338497\\
33	-2.04876892268658\\
34	-1.27710308879614\\
35	-0.734253264963625\\
36	-0.356636513024569\\
37	-0.368397105485201\\
38	-0.431073205545545\\
39	-0.332207512110472\\
40	-0.072698201984167\\
};
%\addlegendentry{$v_{\theta} [rad/s]$}

\end{axis}

\begin{axis}[%
width=4.519in,
height=1.492in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={Step},
ymin=-1.2,
ymax=1.2,
ylabel style={font=\color{white!15!black}},
ylabel={Control},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
title style={font=\huge},xlabel style={font=\LARGE},ylabel style={font=\LARGE},xticklabel style={font=\LARGE},yticklabel style={font=\LARGE}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0515368866328644\\
2	0.119941272967931\\
3	0.207135778240282\\
4	0.311528753180246\\
5	0.422698201395205\\
6	0.525686258210469\\
7	0.612427726321025\\
8	0.683490237468571\\
9	0.744058050322364\\
10	0.799898424519515\\
11	0.85430175993258\\
12	0.906987386132777\\
13	0.955032555087434\\
14	0.992414897673536\\
15	1\\
16	1\\
17	1\\
18	1\\
19	1\\
20	1\\
21	1\\
22	1\\
23	1\\
24	0.833494877422012\\
25	0.388115078317436\\
26	-0.029353027256309\\
27	-0.301655366546425\\
28	-0.449298291928056\\
29	-0.564086286031888\\
30	-0.670165621243957\\
31	-0.759561541016434\\
32	-0.822604042906158\\
33	-0.811097998146217\\
34	-0.740795667994877\\
35	-0.69125475446808\\
36	-0.676736427403139\\
37	-0.645167269401001\\
38	-0.56798599704603\\
39	-0.467140945132063\\
40	-0.397204309683021\\
};
%\addlegendentry{$u_{steer}$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	0.00916885473608718\\
2	0.0163619754641829\\
3	0.0199077338447342\\
4	0.0190840280846646\\
5	0.0151610393549512\\
6	0.0106680490292468\\
7	0.00702316423472026\\
8	0.00395749781804901\\
9	0.000883863666987154\\
10	-0.00227427093840874\\
11	-0.00558191883494476\\
12	-0.0091041275419434\\
13	-0.012324575964207\\
14	-0.0144190142282747\\
15	-0.014694469387976\\
16	-0.0125744532287208\\
17	-0.00749583409654932\\
18	0.000796357731785451\\
19	0.00895064658086157\\
20	0.00429407273095422\\
21	-0.0293754230634645\\
22	-0.0751423870415418\\
23	-0.212317800192824\\
24	-0.395193801720011\\
25	-0.534851437692852\\
26	-0.584625679369643\\
27	-0.548137140951436\\
28	-0.448688298405347\\
29	-0.358428069473606\\
30	-0.294316508567485\\
31	-0.230217096364293\\
32	-0.120633104782169\\
33	0.0221979762671877\\
34	0.16118386037564\\
35	0.257595686462297\\
36	0.334221111144988\\
37	0.39565268589197\\
38	0.382625863055126\\
39	0.244687938137576\\
40	0.132899031650719\\
};
%\addlegendentry{$u_{throttle}$}

\end{axis}
\end{tikzpicture}%

==> figures/scenarios/Parallel_Parking.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00,0.0,1.0}%
\definecolor{mycolor2}{rgb}{1.00,0.0,0.0}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.519in,
height=1.492in,
at={(0.758in,2.553in)},
scale only axis,
xmin=0,
xmax=40,
ymin=-4.2,
ymax=1.2,
ylabel style={font=\color{white!15!black}},
ylabel={Local velocities},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
title style={font=\huge},xlabel style={font=\LARGE},ylabel style={font=\LARGE},xticklabel style={font=\LARGE},yticklabel style={font=\LARGE}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.00154953449964524\\
2	-0.00131450593471527\\
3	-0.0043008103966713\\
4	-0.0095505639910698\\
5	-0.0154877454042435\\
6	-0.0209330767393112\\
7	-0.0253420136868953\\
8	-0.0290673784911633\\
9	-0.0329362973570824\\
10	-0.0374625250697136\\
11	-0.0425238534808159\\
12	-0.0475339964032173\\
13	-0.051637552678585\\
14	-0.0543460808694365\\
15	-0.055946074426174\\
16	-0.0567565485835075\\
17	-0.0563365034759045\\
18	-0.0529989413917065\\
19	-0.0449647195637226\\
20	-0.0357062369585037\\
21	-0.0472356006503105\\
22	-0.0642071664333345\\
23	-0.0384422019124031\\
24	0.00272613018751144\\
25	0.0256270542740822\\
26	0.0125942565500736\\
27	-0.0473035499453544\\
28	-0.158195123076439\\
29	-0.312276966869831\\
30	-0.478777214884758\\
31	-0.617102533578875\\
32	-0.690014138817785\\
33	-0.671886429190635\\
34	-0.563954561948775\\
35	-0.395167395472526\\
36	-0.183102786540985\\
37	0.0092848017811775\\
38	-0.0102859921753407\\
39	0.0091012939810753\\
40	-0.00305106863379478\\
};
%\addlegendentry{$v_{x} [m/s]$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.131190894171595\\
2	-0.344316707924008\\
3	-0.597320683300495\\
4	-0.876112952828405\\
5	-1.16696454584598\\
6	-1.45502060651779\\
7	-1.73064462840557\\
8	-1.99162043631077\\
9	-2.23934501409531\\
10	-2.47558034956455\\
11	-2.7012138068676\\
12	-2.91418768465519\\
13	-3.10499086976052\\
14	-3.27495284378529\\
15	-3.42531703412533\\
16	-3.55770416557789\\
17	-3.6738970130682\\
18	-3.77632409334183\\
19	-3.86898458003998\\
20	-3.95460426807404\\
21	-3.9900840818882\\
22	-3.89149814844132\\
23	-3.76967757940292\\
24	-3.63796703517437\\
25	-3.49026896059513\\
26	-3.31677049398422\\
27	-3.08883480727672\\
28	-2.78323106467724\\
29	-2.42460541427136\\
30	-2.03372061252594\\
31	-1.62704519927502\\
32	-1.22952148318291\\
33	-0.87891384959221\\
34	-0.60074955224991\\
35	-0.384420761838556\\
36	-0.203355671837926\\
37	-0.0764087587594985\\
38	-0.0204447750002146\\
39	-0.000202869996428489\\
40	0.00427591614425183\\
};
%\addlegendentry{$v_{y} [m/s]$}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0011781882494688\\
2	-0.0106602441519499\\
3	-0.0294792372733354\\
4	-0.0503555964678525\\
5	-0.0681828428059815\\
6	-0.0761539209634065\\
7	-0.072219679132104\\
8	-0.0601530354470015\\
9	-0.0443981308490038\\
10	-0.0266433320939541\\
11	-0.00657493248581885\\
12	0.016881488263607\\
13	0.0461218971759081\\
14	0.079383887350559\\
15	0.116048147901892\\
16	0.15845856629312\\
17	0.205525634810329\\
18	0.238457908853889\\
19	0.20857966504991\\
20	0.0740880612283945\\
21	0.00399378128349781\\
22	0.165154477581382\\
23	0.312164062634111\\
24	0.233479058369994\\
25	-0.0420575123280287\\
26	-0.437487568706274\\
27	-0.877775587141515\\
28	-1.29349239170551\\
29	-1.7054994776845\\
30	-2.1018672734499\\
31	-2.4041549116373\\
32	-2.50344313681126\\
33	-2.30303071439266\\
34	-1.79750807583332\\
35	-1.09777104109526\\
36	-0.375937856733799\\
37	0.0459060911089182\\
38	-0.00498502515256405\\
39	0.00137077644467354\\
40	-0.0036423560231924\\
};
%\addlegendentry{$v_{\theta} [rad/s]$}

\end{axis}

\begin{axis}[%
width=4.519in,
height=1.492in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}},
xlabel={Step},
ymin=-0.7,
ymax=1.2,
ylabel style={font=\color{white!15!black}},
ylabel={Control},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
title style={font=\huge},xlabel style={font=\LARGE},ylabel style={font=\LARGE},xticklabel style={font=\LARGE},yticklabel style={font=\LARGE}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	0.409292811215672\\
2	0.632553742193343\\
3	0.725375883392474\\
4	0.768002727535202\\
5	0.794694506033075\\
6	0.816477558673814\\
7	0.837530804837137\\
8	0.859345674194571\\
9	0.88244121523839\\
10	0.907603038726239\\
11	0.936091024818205\\
12	0.968276786492388\\
13	0.998295986430027\\
14	1\\
15	1\\
16	1\\
17	1\\
18	1\\
19	1\\
20	1\\
21	0.926648564275125\\
22	0.575292948248866\\
23	0.367838782065962\\
24	0.268661894019062\\
25	0.194927209980494\\
26	0.101893879398901\\
27	-0.0189178437297904\\
28	-0.126654537719146\\
29	-0.183053577601378\\
30	-0.203300037632671\\
31	-0.210068991547432\\
32	-0.213608996585465\\
33	-0.216731931505627\\
34	-0.220170282072172\\
35	-0.218910149878699\\
36	-0.200248417621064\\
37	-0.155102918211671\\
38	-0.0939650694879363\\
39	-0.0386702586012579\\
40	-0.0200642157262664\\
};
%\addlegendentry{$u_{steer}$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	-0.0218055067585952\\
2	-0.0381144968337034\\
3	-0.048381589801067\\
4	-0.0533003388758291\\
5	-0.0537304375362517\\
6	-0.0504855382256646\\
7	-0.044343131490346\\
8	-0.0360322512652881\\
9	-0.0261481063259167\\
10	-0.0151086167321538\\
11	-0.00320288535397128\\
12	0.0092365272957044\\
13	0.0216651553190571\\
14	0.0339424474452948\\
15	0.0474439734761693\\
16	0.0660268389269916\\
17	0.0929382219453025\\
18	0.116040893529978\\
19	0.0918550622220307\\
20	-0.00674585977129499\\
21	-0.0139423840777843\\
22	0.0945856193147652\\
23	0.0849487437481647\\
24	-0.0176258547155901\\
25	-0.153638948761286\\
26	-0.279133172235829\\
27	-0.363282021638447\\
28	-0.391116402928799\\
29	-0.379239047842487\\
30	-0.351771295991313\\
31	-0.324901697022686\\
32	-0.304401422217401\\
33	-0.289255918946309\\
34	-0.276182385555196\\
35	-0.262165921307073\\
36	-0.245680881417727\\
37	-0.232853979693184\\
38	-0.233427492991211\\
39	-0.223028365398283\\
40	-0.169812714355707\\
};
%\addlegendentry{$u_{throttle}$}

\end{axis}
\end{tikzpicture}%
